Drell-Yan cross-sections with fiducial cuts: impact of linear power corrections and $q_T$-resummation in PDF determination

Measurement at Hadron colliders of neutral- and charged-current Drell-Yan production provide essential constraints in the determination of parton distribution functions. Experimentally, they have reached percent level precision, challenging the accuracy of the theoretical predictions. In this work we benchmark the novel implementation in $\texttt{DYTurbo}$ of linear fiducial power corrections in the $q_T$-subtraction formalism at NLO and NNLO in QCD. We illustrate how the inclusion of linear fiducial power corrections impacts predictions for precise $W$ and $Z$ measurements from the LHC and affects their description by modern global parton distribution functions. The further inclusion of $q_T$-resummation corrections in the theoretical predictions leads to a better modelling of the lepton $p_T$ distribution and we study how this improve the description of the data.

==> pheno-study.tex <==
\newcommand{\obs}{\mathcal{O}} 
\newcommand{\sigmahat}{\hat{\sigma}} 
\newcommand{\taucut}{\tau_{cut}}
\newcommand{\dsigmadtau}{\frac{d\sigma}{d\tau}}
\newcommand{\dsigmadtauup}[1]{\frac{d\sigma^{#1}}{d\tau}}
\newcommand{\ptl}{p_{T,\,\ell}}
\newcommand{\etal}{\eta_{\ell}}
\newcommand{\mll}{m_{\ell\ell}}
\newcommand{\absyll}{|y_{\ell\ell}|}
\newcommand{\de}{\text{d}}
\newcommand{\sigmaR}{\sigma^{\text{R}}}
\newcommand{\sigmatext}[1]{\sigma^{\text{#1}}}
\chapter{High precision Drell-Yan predictions}\label{chap:pheno-study}
The level of accuracy reached by the high energy physics experiments imposes the need for high precision in the theoretical predictions. The prime process for precision benchmarking is the Drell-Yan process, this can be both measured and predicted with high accuracy. The calculation needs to take into account extra radiation in the final state and the most important contribution comes from QCD radiation. The experimental results are often extracted within the fiducial region, that corresponds to the application of kinematic cuts on the final state leptons. For a meaningful comparison with the experimental data, the prediction must also implement fiducial cuts. To do this the fully exclusive cross-section for the vector boson production is needed. This is known up to NNLO in QCD for Drell-Yan process \cite{nnlo-exclusive-dy-catani,nnlo-dy-fewz,nnlo-dy-mcfm}. 
%The state of the art precision of QCD calculation ims NNLO (order $\alpha_S$) is QCD. 
The NNLO calculation considers up to two additional emissions and must deal with the cancellation of the related soft and collinear singularities. To this purpose two main approaches have been developed. These are often referred to as \emph{slicing} and \emph{local} singularity subtraction schemes. Thanks to the success of these methods,  the NNLO QCD accuracy for DY is now the state of the art and the predictions can be obtained with various public codes \cite{nnlo-dy-fewz,nnlo-dy-mcfm,MATRIX-dy-nnlo,dyturbo}. More recently also inclusive N3LO results have been obtained \cite{dy-n3lo}.
Despite the level of precision claimed by the NNLO codes, it has been noticed that the results differ between each other by an amount that can reach the percent level. This has been noticed for example by the ATLAS collaboration in performing the $W/Z$ cross section measurement at $7\umeas{TeV}$ \cite{atlas-w-z-7tev}. The disagreement is understood to be related to the presence of fiducial cuts applied to final state leptons and the different subtraction schemes adopted in the calculation \cite{fpc-tackman,moch-benchmark-nnlo}. The disagreement can be as high as few percent, in some cases this is of the same order as the pure NNLO correction term and, most importantly, is not negligible compared to the experimental uncertainty of some DY measurements. In the case of the ATLAS $W/Z$ measurement mentioned above, for example, the maximum precision reached is of $0.5\%$. These differences in the theory predictions can have an impact on PDF extraction where Drell-Yan differential measurements play an important role in constraining the $u-$ and $d-$quark valence distributions.

In this chapter a benchmark study of predictions for the DY process produced with different codes adopting different subtraction schemes is reported. In section \ref{sub-methods} the idea behind the different subtraction approaches is described. In section \ref{sec:fiducial-power-corr} the problem of linear power correction that biases the results of slicing methods, in the presence of fiducial cuts, is explored. The results of the benchmark comparison are reported in section \ref{sec:nlo-nnlo-benchmark}. The predictions are produced in the fiducial region used in the ATLAS $W/Z$ $7\umeas{TeV}$ cross section measurement \cite{atlas-w-z-7tev}. The same calculations are used in section \ref{sec:pdf-study} for a PDF study where the agreement of the predictions in combination with different PDFs and the data is assessed.


\section{Subtraction methods}\label{sub-methods}
In section \ref{sec:high_order_qcd}, Figure \ref{fig:dy-nlo}, the different diagrams contributing to the NLO QCD correction for the DY process were presented; in general, two kind of terms are identified: virtual loop correction to the LO vertex and real emission correction. Both contributions present collinear and soft (or infrared (IR)) singularities. General results guarantee the cancellation of the IR singularity when summing up the two contribution \cite{Lee-Nauenberg,kinoshita}, and the universal factorisation of the collinear poles, that can be absorbed into a renormalization of the PDFs. These results are valid at each perturbative order. At NNLO the classes of divergent contributions are three: double real emission, real-virtual contribution, and double loop correction. Despite the cancellation of the IR singularities the problem of calculating the exclusive cross section is challenging: fully analytical results for a general  phase space integration are not available and numerical results cannot be applied straightforwardly due to the divergent nature of the integrand. In the virtual and real correction terms, the number of final state particles is different, and the phase space integration has to be performed separately, preventing direct cancellation in the sum of the two terms. Two classes of techniques, \emph{local subtraction} and \emph{slicing} methods, have then been developed to isolate and regularize the divergent terms in the integrands. In the next sections  the idea behind the two methods is presented.

\subsection{Slicing methods}\label{sec:slicing-methods}
Slicing methods identify an IR safe observable that resolves additional emissions. This observable is used to slice the phase space integration into two regions, one containing the singular term and the other in which the cross section is regular. The regular part can be integrated safely using standard techniques, the singular part is instead approximated thanks to the known universal structure of the singularities.

Typical observables are the transverse momentum $q_T$ of a color singlet \cite{nnlo-exclusive-dy-catani},\cite{nnlo-exclusive-higgs-catani} and N-jettiness \cite{tackmann-njettiness}. In the Drell-Yan process $q_T$ is the transverse momentum of the vector boson. The slicing parameter is usually defined as 
\begin{equation}
    \tau = \frac{q_T^2}{Q^2} 
\end{equation}
 $Q^2$ is the hard scale of the born level process, the invariant mass of the exchanged boson in the DY case. When $\tau\rightarrow 0$ the cross section $d\sigma/d\tau$ reaches the singular limit. The cross section integration is sliced by introducing a threshold value $\tau_{\text{cut}}$
\begin{equation}\label{eq:cross-sec-slicing}
    \sigma = \int_0^{\tau_{\text{cut}}} \de\tau \frac{\de\sigma}{\de\tau} + \int_{\tau_{\text{cut}}}\de\tau  \frac{\de\sigma}{\de\tau} 
\end{equation}
The first term in the right hand side contains the singular term, while the second term is regular and can be integrated with standard techniques. The integrand, $d\sigma/d\tau$, can be divided into two contributions, the singular one, that contains the singular contribution as  $\tau\rightarrow0$ and a non-singular one
\begin{equation}
    \dsigmadtau = \dsigmadtauup{\text{sing}} +  \dsigmadtauup{\text{nonsing}}.
\end{equation}
The slicing method relies on the fact that the singular contribution, that dominate the low $\tau$ integration part, can be predicted from the factorisation theorem, the structure of the IR singularities and the KLN theorem. The structure is of the type 
\begin{equation}\label{eq:xs-singular}
    \frac{d\sigma^{\text{sing}}}{d\tau} \sim \delta(\tau) + \sum_i \left[ \frac{\ln\tau}{\tau} \right]_+
\end{equation}
The $+$ distribution, whose definition was given in equation \ref{eq:plus-distribution}, indeed represents the structure of the cancellation between the real and virtual IR divergences. This knowledge can be used to approximate the cross section at low $\tau$. Integrating the singular term up to the threshold $\taucut$ one obtains something of the order
\begin{equation}\label{eq:xs-singular-integrated}
    \sigma^{\text{sing}}(\taucut) = \int_0^{\taucut} \frac{d\sigma^{\text{sing}}}{d\tau} \sim 1 + \sum_{j\geq0} \ln^{j+1}\tau_{\text{cut}}.
\end{equation}
$\sigma^{\text{nonsing}}$ instead includes terms that are at least $\tau$ integrable, or that go to zero when $\tau\rightarrow 0$. The structure is of type 
\begin{equation}\label{eq:xs-nonsingular}
\begin{split}
     &\dsigmadtauup{\text{nonsing}} \sim \sum_{m>0} \sum_{j\geq 0} \tau^{m-1}\ln^{j}\tau \\  &\sigma^{\text{nonsing}}(\tau_{\text{cut}}) = \int_0^{\tau_{\text{cut}}} d\tau \dsigmadtauup{\text{nonsing}} \sim \sum_{m>0} \sum_{j\geq 0} \tau^{m}\ln^{j}\tau \sim O(\tau)
\end{split}
\end{equation}
These are considered power corrections ($O(\tau_{\text{cut}}^m),\,m>0$) to the singular term.
The cross section in eq. \ref{eq:cross-sec-slicing}  is calculated by adding and subtracting a subtraction term $\sigma^{sub}$
\begin{equation}\label{eq:cross-sec-sigmasub}
    \sigma = \sigma^{sub} (\tau_{\text{cut}}) + \int_{\tau_{\text{cut}}} d\tau \frac{d\sigma}{d\tau} + \Delta\sigma^{sub}(\tau_{\text{cut}}).
\end{equation}
 $\sigma^{sub} (\tau_{\text{cut}})$ approximates the cross section at low $\tau$, while
the term $\Delta\sigma^{sub}(\tau_{\text{cut}}) = \sigma(\tau_{\text{cut}}) - \sigma^{sub}(\tau_{\text{cut}})$, that is neglected when doing the computation, represents the error of this approximation. $\sigma^{sub} (\tau_{\text{cut}})$ should include at least the singular term of equation \ref{eq:xs-singular-integrated},
\begin{equation}
    \sigma^{sub}(\taucut) = \sigma^{\text{sing}}(\taucut) [1 + O(\tau_{\text{cut}})]
\end{equation}
so that the error in the calculation is a power correction
\begin{equation}\label{eq:delta-sigma-power-corr}
    \Delta\sigma^{sub}(\tau_{\text{cut}}) \sim O(\tau^m_{\text{cut}})
\end{equation}
The actual value of $m$ depends on how many terms of $\sigma^{\text{nonsing}}(\tau_{\text{cut}})$, equation \ref{eq:xs-nonsingular}, can be included in $\sigma^{sub}$. In the case of the inclusive Drell-Yan cross section the $O(\tau^1_{\text{cut}})$ is known at NLO and can be included in $\sigma^{sub}$. The neglected term $\Delta \sigma$ is a power correction $O(\tau^2_{\text{cut}})$. The presence of fiducial cuts on the final state leptons can introduce additional power dependence of $\de\sigma^{\text{nonsing}}/\de\tau$ on $q_T$ and lower the precision of the approximation.

\subsection{Fiducial power corrections}\label{sec:fiducial-power-corr}
The power corrections to the singular term, equation \ref{eq:xs-nonsingular}, represent the intrinsic error of slicing subtraction methods. This error is of order $O((q^2_{T,\, \text{cut}}/Q^2)^2)$ in the case of DY predictions and for inclusive calculation. A choice of the slicing threshold $\tau_{\text{cut}}=(q^2_{T,\, \text{cut}}/Q^2)$ small enough makes this bias negligible. The presence of fiducial cuts on the final state leptons, however, can introduce additional power $q_T$ correction that cause a further bias in the predictions. These fiducial power corrections (FPC) arise when considering the final state phase space integration. Using a schematic notation, the phase space integration reads as
\begin{equation}
    \dsigmadtau = \int d\Phi_F \dsigmadtau(\Phi_F)
\end{equation}
where $d\Phi_F$ represent the phase space integration on the final state leptons. The singular term of the cross section depends only on the Born phase space, where no additional emission are considered, 
\begin{equation}
    \dsigmadtauup{\text{sing}} = \int d\Phi^{\text{Born}}_F \dsigmadtauup{\text{sing}}(d\Phi).
\end{equation}
When applying fiducial cuts a dependence of the acceptance, $\Phi_F = \int d\Phi_F$, on the boson transverse momentum is introduced. The reason is shown intuitively in Figure \label{fig:fpc-sketch}  where the $p_T$ cut on the leptons coming from the $Z$ decay are shown schematically. When the $Z$ is at rest both leptons pass the requirement $p_{T\,1,2}>p_T^{\text{min}}$. 
This is no longer the case when the $Z$ boson is given a small transverse momentum. 
\begin{figure}
    \centering
    \includegraphics[width = 0.95\textwidth]{pheno-study/fid-power-correction-sketch.pdf}
    \caption{Schematic representation of the rising of $q_T$ power corrections due to fiducial cuts on the final state leptons. On left, the case in which the $Z$ boson is at rest and the two lepton are passing the fiducial cuts is shown. When the $Z$ is given a small transverse boost, Figure on the right, one of the two leptons fail to pass the selection.}
    \label{fig:fpc-sketch}
\end{figure}
The error introduced in the slicing method can be estimated by comparing the acceptance of the final state with the Born one
\begin{equation}
    \Delta \Phi_F = \int d\Phi_F(q_T) - d\Phi_F^{\text{Born}}(q_T = 0)
\end{equation}
It has been shown \cite{fpc-tackman} that 
\begin{equation}
    \Delta \Phi_F \sim \frac{1}{q_T^2}\left(\frac{q_T^2}{Q^2}\right)^m
\end{equation}
where the value of $m$ depends on the fiducial cut configuration. In the case of a $p_T^{\ell}$ symmetric cut, $p_{T}^{\ell_1,\,\ell_2}>p_T^{\text{min}}$, it is found that $m=1/2$, that means
\begin{equation}
    \left.\Delta \Phi_F\right|_{p_{T}^{\ell_1,\ell_2}>p_T^{\text{min}}} \sim \frac{1}{q_T^2}\left(\frac{q_T}{Q}\right)
\end{equation}
This linear dependence introduces a bias in the cross section calculation, equation \ref{eq:cross-sec-sigmasub}, that is dominant with respect to the inclusive power corrections, equation \ref{eq:delta-sigma-power-corr}. In the case of additional lepton pseudorapidity cuts, for example a symmetric cut $|\eta_{\ell_1,\ell_2}|< \eta_{\text{min}}$, linear power correction also arise, but effects can be different according to the di-lepton rapidity configuration.  A more detailed analysis of the relation between different fiducial cut configurations and the power corrections can be found in Refs \cite{moch-benchmark-nnlo,salam-two-body-decay}.

A simple solution in the DY case to avoid this bias is to change the selection configuration. A selection in which different cut thresholds are applied to on the lepton and anti-lepton $p_T$, also known as \emph{staggered} cuts, is not affected by linear $q_T$ biases \cite{matrix-fully-diff-NNLO,salam-two-body-decay}. 
The symmetric cuts are anyway still common in DY measurements and relevant measurements have been performed with this configuration \cite{atlas-w-z-7tev}. A way to mitigate the effects of the linear power corrections is then needed.
A first possibility is to lower the $q_{T,\,\text{cut}}$ threshold value, or to have an extrapolation method to small $q_{T,\,\text{cut}}$ values. Both of these approaches affect the stability and the performance of the calculation. Furthermore the  introduction of a dependence of the cross section on $q_T$ introduces some instability in the series expansion due to non perturbative small-$q_T$ effects \cite{salam-two-body-decay}. These affect any fixed order calculations, regardless of the subtraction scheme. A more feasible approach is then to include the $q_T$ resummation effects in the predictions. It has been shown in Ref. \cite{tackman-fpc-resummation} that the implementation of a recoil prescription of the boson transverse momentum as done in the $q_T$ resummation \cite{pt-resum-catani-2015,pt-resum-becher,pt-resum-bertone-2019,n3ll-radish,n3ll-wan-li-ju-2020,dyturbo}, allows the linear power corrections to be resummed at each perturbative order. The residual fiducial biases are quadratic in $q_T$ and so of the same order as in the inclusive case. Starting from this result it is also possible to include the linear power correction in $q_T$ at a given order in $\alpha_S$. This gives a fixed order result that can be used for a benchmark study with the local subtraction method predictions.
This procedure has been implemented in public code such as MATRIX \cite{matrix-fpc} or DYTurbo \cite{dyturbo-fpc}. In section  \ref{sec:nlo-nnlo-benchmark} a benchmark study of predictions for the DY process in the case of fiducial cuts is presented and the DYTurbo code is used. 

%By considering a lower cut value $\obs_{cut}>\obs_0$ it is possible to individuate two different regions: one that is finite ($\obs < \obs_{min}$) and can be safely integrated with standard techniques, over the $N+1$ particles phase space and the remaining region ($\obs < \obs_{min}$), that contain the singularity.   
%In this region the singular contribution factorize and the finite part of the integrand is approximated by a regular function $
%\mathcal{F}$. The integral is now over a $N$ particle phase space and can be combined with virtual contribution. At NLO the procedure can be written schematically as 
%\begin{equation}
%    \hat{\sigma}^{\text{NLO}} = \int_{\Phi_{N+1}} d\sigmahat^{\text{Real}} \,\Theta(\obs-\obs_{cut}) + \int_{\Phi_{N}} d\mathcal{F} + \int_{\phi_{N}} d\sigma^{\text{Virtual}}|_{\obs = \obs_0}
%\end{equation}
%%where 
%\begin{equation}
%    \int_{\Phi_{N+1}} d\sigmahat \,\Theta(\obs_{cut}-\obs) \sim \int_{\Phi_{N}} d\mathcal{F}
%%\end{equation}
%Typical observable used in slicing methods are the transverse momentum $q_T$ of a color singlet \cite{nnlo-exclusive-dy-catani},\cite{nnlo-exclusive-higgs-catani}, the vector boson transverse momentum in the DY case and the N-jettiness. The result should be independent of $\obs_{cut}$, in reality a small dependence remains. This can be reduced by reducing the value of $\obs_{cut}$ even though this increase drastically the computation time and the introduce instability problems.

\subsection{Local subtraction methods}
The other strategy to deal with the divergences is the local subtraction method. This aims to correct for the singular contributions in the cross section point by point at the integrand level, so that the phase space integration can be freely performed, without the need of approximations. In the case of NLO calculations, the cross section can be split into the real and virtual contributions, whose phase space integration is performed over a different number of particles in the final state
\begin{equation}
    \sigma^{NLO} = \int d\sigma = \int_{N+1}d\sigma^{\text{R}} + \int_{N} d\sigma^{V}
\end{equation}
A subtraction for the real term that encodes all its IR divergences is now constructed. Adding it to the real term eliminates the singularities, so that the $N+1$ phase space integration can be performed
\begin{equation}
\begin{split}
    \sigma^{NLO} &= \int_{N+1} \de \sigmaR - \int_{N+1} \de \sigmatext{S} + \int_{N+1} \de \sigmatext{S} + \int_{N} \de \sigmatext{V} \\
    &=\int_{N+1} \left[\de \sigmaR -  \de \sigmatext{S}\right] + \int_{N+1} \de \sigmatext{S} + \int_{N} \de \sigmatext{V}
\end{split}
\end{equation}
The subtraction term is also built in a way that the integral on the extra particle can be factorized and the term can be combined with the virtual contribution. In particular it can be combined with the loop integral in the virtual term from which the infrared singularity arises, hence allowing the cancellation
\begin{equation}
    \sigma^{NLO} = \int_{N+1} \left[\de \sigmaR -  \de \sigmatext{S}\right] + \int_{N} \left[ \int_{\text{loop}} \de \sigmatext{V} + \int_{1} \de \sigmatext{S} \right].
\end{equation}

The definition of the subtraction term presents a certain freedom, in particular in its finite contribution. Different definition choices is what distinguish the local subtraction methods available for the calculation. At NLO the FKS \cite{nlo-FKS-sub-scheme} and the Catani-Seymour \cite{nlo-catani-seymur-sub-scheme} schemes are implemented. At NNLO the level of complexity is significantly higher due to the overlapping of singularities. One of the established method is antenna subtraction \cite{antenna-nnlo,antenna-nnlo-hadronic,antenna-nnlo-infrared}, this is implemented in the NNLOJET code. NNLO Drell-Yan predictions from this program are used in the next section for the benchmark study. 

An alternative approach is the \emph{sector decomposition}  as implemented in the simulation code FEWZ \cite{nnlo-dy-fewz}  or in the STRIPPER code \cite{stripper-I,stripper-II,stripper-III}.
%, projection to Born \cite{projection-to-bornI,projection-to-bornII}, ColorfulNNLO \cite{colorfull-I,colorfull-II}.

\section{NLO and NNLO benchmark study}\label{sec:nlo-nnlo-benchmark}
In this section a benchmark study of NLO and NNLO QCD predictions for the DY process is presented. The comparison is performed between the results of two codes: DYTurbo and NNLOJET. These use different subtraction schemes, DYTurbo implements a slicing subtraction in $q_T$ \cite{dyturbo}, while NNLOJET uses a local subtraction based on the antenna subtraction method. A treatment to include the linear $q_T$ power corrections due to the fiducial cuts is implemented in DYTurbo \cite{dyturbo-fpc} and is benchmarked in this section. Furthermore, the DYTurbo offers also the possibility to include the $q_T$ resummation effects in the predictions. Also these predictions are used in the comparison. The benchmark is performed in the context of predictions for the ATLAS $7\umeas{TeV}$ $W/Z$ measurement. This offers an interesting case in which to evaluate the differences in the theory as this data set reaches an high experimental precision and contributes significantly in the PDF determination. The same predictions will be used in section \ref{sec:pdf-study} for a comparison of the different theory definitions with the data.

\subsection{Fiducial region}\label{sec:fiducial-region}
The predictions are produced in the fiducial region of the ATLAS $7\umeas{TeV}$ $W/Z$ cross section measurement \cite{atlas-w-z-7tev}. Only the $Z/\gamma^*\rightarrow \ell\ell$ cross section is used in the benchmark study.

The ATLAS measurement is performed in two channels. A central channel that selects leptons at central pseudorapidity, $|\eta_{\ell}|<2.5$, and a forward channel in which one of the two leptons is required to be produced at high pseudorapidity, $2.5<|\eta_{\ell}|<4.9$. The kinematics requirement applied for the cross section measurement are
\begin{equation}
    \begin{split}
        \text{Central}\,\, Z/\gamma^*\rightarrow\ell\ell:\,\,& \ptl>20\umeas{GeV},\\
        &|\etal|<2.5,\\
        &46<\mll<150\umeas{GeV}\\
        \text{Forward}\,\, Z/\gamma^*\rightarrow\ell\ell:\,\,& \ptl>20\umeas{GeV},\\
        & \text{one lepton}\,|\eta|<2.5,\, \text{the other lepton}\,\, 2.5<|\eta|<4.9,\\
        & \,66<\mll<150\umeas{GeV}
    \end{split}
\end{equation}
The cross section is measured in three different bins of the dilepton invariant mass
\begin{equation}
    m_{\ell\ell} = [46, 66, 116, 140]\umeas{GeV}
\end{equation}
these are referred to as \emph{low mass}, \emph{$Z$-peak} and \emph{high mass} bins. In the low mass bin only the central channel is measured. In each mass bin the cross section is measured differentially in the dilepton rapidity $\absyll$. In the $Z$-peak region, central channel, the following bins edges are used
\begin{equation}
    \absyll = [0.0, 0.2, 0.4, 0.8, 1.0, 1.2, 1.4, 1.6, 1.8, 2.0, 2.2, 2.4]
\end{equation}
In the low and high mass bins a binning twice as coarse is used. When measuring the cross section in the forward channel instead, bins with the following boundaries are chosen
\begin{equation}
    \absyll = [1.2, 1.4, 1.6, 1.8, 2.0, 2.2, 2.4, 2.8, 3.2, 3.6].
\end{equation}

The same fiducial region and binning schemes are used in producing the predictions. The measurement implements symmetric cuts on the lepton and anti-lepton $p_T$ and both asymmetric and symmetric cuts (according to the channel) on the lepton pseudorapidity $\eta$. As discussed in section \ref{sec:fiducial-power-corr}, an increase in the fiducial power correction when calculating the cross section with slicing subtraction methods is expected in all these configuration .

\subsection{Simulation setup}
The DYTurbo and NNLOJET prediction are calculated with the same input parameters.
The $G_{\mu}$ scheme is used:  $G_F$, $m_W$, $m_Z$ are the input values while $\sin^2\theta_W$ and the QED coupling $\alpha(m_Z)$ are calculated as output. In general, the Standard Model input parameters are set to the following values \cite{PDG}
\begin{equation}
    \begin{split}
        G_F &= 1.1663787\times10^{-5}\umeas{GeV}^{-2},\\
        m_Z &= 91.1876 \umeas{GeV},\\
        m_W &= 79.936 \umeas{GeV}, \\
        \Gamma_Z &= 2.4950\umeas{GeV}, \\
        \Gamma_W &= 2.091 \umeas{GeV}. \\
    \end{split}
\end{equation}
The CKM matrix elemets are set to \cite{PDG}
\begin{equation}
  \begin{alignedat}{2}
        |V_{ud}| &= 0.97427, \quad & & |V_{cd}| = 0.2252, \\
        |V_{us}| &= 0.2253, \quad  & & |V_{cs}| = 0.97344, \\
        |V_{ub}| &= 0.00351, \quad & & |V_{cb}| = 0.0412 \\
  \end{alignedat}
\end{equation}
The input PDFs are taken from the NNPDF3.1 set \cite{nnpdf31}. The values of the renormalization and factorization scale $\mu_R$ and $\mu_F$ is set to in the dilepton invariant mass in each event, $\mu_R=\mu_F=\mll$. 

DYTurbo implements a slicing subtraction scheme in $q_T$. The vaule of the slicing cut-off is set to $(q_T/Q)_{\text{cut}} = 0.008$. Additional parameters to include the resummation effects need to be set. The first is the resummation scale $\mu_{\text{Res}}$ that is set, as the renormalization and factorization scales, to the dilepton invariant mass $m_{\ell\ell}$. The resummation damping function that regulates the vanishing of the resummation effects at high $q_T$ is set to a Gaussian: $f(x) = \exp(-(k\,m_{\ell\ell}-q_T)^2/\Delta\,m_{\ell\ell}^2)$ with $k=0.75$ and $\Delta = 0.5$. A term to parametrize non-perturbative QCD effects also needs to be included. This is a Gaussian form factor in the space of the impact parameter $b$, $G^\text{{NP}}(b) = \exp(-g_1 b^2)$ with $g_1=0.8$.

A comparison of the predictions at LO, where no difference due to the subtraction schemes is expected, is carried out to test the simulation setup. Agreement at the level of 0.1per mille is found.

\subsection{NLO comparison}
The predictions at NLO QCD are compared. DYTurbo implements the $q_T$ slicing also at this perturbative order and differences with respect to the NNLOJET results are expected. The fiducial power correction term implemented in DYTurbo is considered, this helps to recover good agreement between the two subtraction scheme calculations.

In figure \ref{fig:nlo-comp-zypeak-cc-cf} the NLO comparison for the $Z$-peak bin predictions, in the central and forward channel is shown. A disagreement beetween the fixed order DYTurbo and NNLOJET results is observed. In the central channel the differences are of the order of 6 per mille, these are more severe in the forward channel where the ratio departs from one as much as $7\%$. The inclusion of the FPC term in the DYTurbo predictions improves the agreement at the level better than $0.5$ per mille. Similar observation can be made by comparing the predictions in the high mass bin, Figure \ref{fig:nlo-comp-zyhigh-cc-cf}. The effect of fiducial cuts are partially smaller than in the $Z$-peak bin and again, adding the FPC term to the DYTurbo predictions, increases the agreement at a per mille level.  In the low mass bin \ref{fig:nlo-comp-zylow-cc} the effect of using different subtraction methods results only in a 2 per mille difference at central rapididty, including the FPC further improves the agreement.
\begin{figure}
    \centering
    \includegraphics[width = 0.49\textwidth]{pheno-study/nlo-comparison/zypeak_cc.pdf}
    \includegraphics[width = 0.49\textwidth]{pheno-study/nlo-comparison/zypeak_cf.pdf}
    \caption{NLO QCD predictions for the ATLAS $Z$-peak central (left) and forward (right) channel. The fixed order DYTurbo prediction shows a disagreement with respect to the NNLOJET. Good agreement is recovered after including the FPC term.} \label{fig:nlo-comp-zypeak-cc-cf}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width = 0.49\textwidth]{pheno-study/nlo-comparison/zyhigh_cc.pdf}
    \includegraphics[width = 0.49\textwidth]{pheno-study/nlo-comparison/zyhigh_cf.pdf}
    \caption{NLO QCD predictions for the ATLAS high mass central (left) and forward (right) channel. The fixed order DYTurbo prediction shows a disagreement with respect to the NNLOJET is observe. Good agreement is recovered after including the FPC term. In the forward channel some residual discrepancies are observed at very high rapidity.}
    \label{fig:nlo-comp-zyhigh-cc-cf}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = 0.49\textwidth]{pheno-study/nlo-comparison/zylow_cc.pdf}
    \caption{NLO QCD predictions for the ATLAS low mass central channel. The fixed order DYTurbo prediction is in slight disagreement with respect to the NNLOJET. Including the FPC term the agreement is further improved.}
    \label{fig:nlo-comp-zylow-cc}
\end{figure}

\subsection{NNLO comparison}
A benchmark study at NNLO precision is performed in this section. In the comparison, also the DYTurbo results that include the $q_T$ resummation corrections are reported, as they will be used in the next section for the PDF study. These prediction correspond to a NNLO+NNLL accuracy. In Figure \ref{fig:nnlo-zypeak-cc-cf} the comparison of the NNLO $Z$-peak bin predictions is reported. Both in the forward and central channel differences between NNLOJET and the fixed order DYTURBO results are observed. These are of the the same order as those noticed at NLO, Figure \ref{fig:nlo-comp-zypeak-cc-cf} (but in the opposite direction: at NLO DYTurbo undershoots the NNLOJET cross section, here it overshoots it). Adding the FPC term, DYTurbo is able to recover a per mille level agreement. The NNLO+NNLL result deviates from the fixed order by few per mille in the central channel, with some shape differences for $\absyll>1.2$. In the forward channel the resummation seems to have a bigger effect, and the deviation gets as high as $3\%$.

\begin{figure}
    \centering
    \includegraphics[width = 0.49\textwidth]{pheno-study/nnlo-comparison/zypeak_cc.pdf}
    \includegraphics[width = 0.49\textwidth]{pheno-study/nnlo-comparison/zypeak_cf.pdf}
    \caption{Comparison of the NNLO QCD calculations from NNLOJET and DYTURBO. The predictions are for the $Z$-peak bin in the central (left) and forward (right) channel.}
    \label{fig:nnlo-zypeak-cc-cf}
\end{figure}

In the high mass bin, Figure \ref{fig:nnlo-zyhigh-cc}, the inclusion of the FPC term doesn't improve the agreement of the DYTurbo results with the NNLOJET ones. For both in the central and forward it actually slightly increases the differences. The reason for this behaviour is yet to be understood. The resummation effects lead to few per mille deviations in the central channel and up to per cent differences in the forward channel.

\begin{figure}
    \centering
    \includegraphics[width = 0.49\textwidth]{pheno-study/nnlo-comparison/zyhigh_cc.pdf}
    \includegraphics[width = 0.49\textwidth]{pheno-study/nnlo-comparison/zyhigh_cf.pdf}
    \caption{Comparison of the NNLO QCD calculations from NNLOJET and DYTURBO. The predictions are for the high mass bin in the central (left) and forward (right) channel.}
    \label{fig:nnlo-zyhigh-cc}
\end{figure}

The comparison for the low mass bin predictions is reported in Figure \ref{fig:nnlo-zylow-cc}. An improvement in the agreement when including the FPC term is observed this time. The differences are reduced to a $5$per mille level. The resummed DYTurbo result has a shape similar to the fixed order one, but a $2.5\%$ offset difference.
\begin{figure}
    \centering
    \includegraphics[width = 0.55\textwidth]{pheno-study/nnlo-comparison/zylow_cc.pdf}
    \caption{Comparison of the NNLO QCD predictions for the low mass bin.}
    \label{fig:nnlo-zylow-cc}
\end{figure}

\section{Data theory comparison}\label{sec:pdf-study}
Thanks to the experimental precision and the wide phase space considered, the ATLAS data presented in section \ref{sec:fiducial-region} provide a significant constraint on the PDFs \cite{atlas-w-z-7tev}. These measurements are usually included in determining modern PDF sets. In this section a study of the compatibility of some modern PDF sets with the ATLAS data when changing the underlying theory is reported. The study is performed with \emph{xfitter} \cite{xfitter}, an open source software that offers a framework for PDF determination.

%\subsection{PDF determination}

%The profiling procedure \cite{pdf-profiling,pdf-profile-nlo-camarda} is originally though as a way of testing the impact of new data set in the PDF determination. Given a PDF set, the profile furnish a test of compatibility between the PDFs and the data set under study, within the PDF and experimental errors. Here the procedure is used to test the compatibility when using the different definitions of NNLO QCD calculations presented in the previous section.
The data theory compatibility is carried out through a $\chi^2$ test. The $\chi^2$ definition takes into account the correlated systematic uncertainties, both experimental and theoretical (from the PDFs), introducing nuisance parameters that are extracted through a $\chi^2$ minimization. The $\chi^2$ at the minimum is equivalent to the more standard definition $\chi^2 = \sum_{ij} (\sigma^{\text{exp}}_i - \sigma^{\text{th}}_j) V^{-1}_{ij} (\sigma^{\text{exp}}_j - \sigma^{\text{th}}_j)$, where $V_{ij}$ is the uncertainty covariance matrix, see Ref. \cite{correlated-syst-chi2,chi2-pdfUncert-lagrangianMul} for the proof. Using the nuisance parameter approach is computationally more feasible because one avoids the inversion of the matrix $V_{ij}$. Furthermore it allows us to distinguish between the different sources of systematics. The $\chi^2$ is defined as
\begin{equation}\label{eq:prof-chi2}
\begin{split}
    \chi^2(\mathbf{b}_{\text{exp}}, \mathbf{b}_{\text{th}}) =&  \sum_{i=1}^{N_{\text{data}}} \frac{\left[\sigma^{\text{exp}}_i - \sigma^{\text{th}}_i(1 - \sum_k\gamma_{ik}^{\text{th}}b_{k,\text{th}} - \sum_j\gamma_{ij}^{\text{exp}}b_{j,\text{exp}} )\right]^2}{\Delta_i^2} \\
        & +  \sum_i \log \frac{\delta^2_{i,\text{uncor}}(\sigmatext{th}_i)^2 + \delta^2_{i,\text{stat}}\sigmatext{exp}_i\sigmatext{th}_i}{\delta^2_{i,\text{uncor}}(\sigmatext{exp}_i)^2 + \delta^2_{i,\text{stat}}(\sigmatext{exp}_i)^2} \\
    & + \sum_{j=1}^{N_{\text{exp.sys}}}b^2_{j,\text{exp}} + \sum_{k=1}^{N_{\text{th.sys}}} b^2_{k,\text{th}}.
\end{split}
\end{equation}
In the formula, the index $i$ runs over all $N_{\text{data}}$ points.
For each point, the data measurement $\sigma_i^{\text{exp}}$ and theory point $\sigma_i^{\text{th}}$ are compared taking into account both the experimental uncertainties and theoretical uncertainties coming from PDF variations. The uncorrelated experimental uncertainties are given by $\Delta_i$. The correlated uncertainty component is included introducing the nuisance parameter vectors $\mathbf{b_{\text{exp}}}$ and $\mathbf{b_{\text{th}}}$. The impact of the uncertainty source $j$ on the data(theory) point $i$ is described by the matrices $\gamma^{\text{data(th)}}_{ij}$ . Both the correlated and uncorrelated uncertainties are treated as multiplicative (the uncertainties are proportional to central prediction values). The $\chi^2$ function is minimized as a function of $\mathbf{b_{\text{exp}}}$ and $\mathbf{b_{\text{exp}}}$. The contribution to the $\chi^2$ for the determination of the nuisance parameters is given by the two sums of $b^2_{j}$ over the number of correlated uncertainty sources $N_{\text{exp.sys}}$, $N_{\text{th.sys}}$. This term is referred to as \emph{correlated $\chi^2$} contribution when reporting the results of the study. The $\log$ term instead is added to minimize biases. Because the $\chi^2$ is quadratic in $\mathbf{b}$ the minimization can be performed analytically. The $\chi^2$ at its minimum gives a test of compatibility between data and theory. The values of the nuisance parameters $b_{k,\,\text{th}}$ at this minimum can be interpreted as an optimization of the PDFs to describe the data, and allows us to determine a new set of PDFs. This procedure is called PDF profiling \cite{pdf-profiling,pdf-profile-nlo-camarda} and can be used to test in a quantitative way the impact of new data measurement on a PDF set  without performing a new PDF fit.  In this study we limit our self to use the $\chi^2$ at the minimum as a way to check the agreement with the data. The theory points $\sigmatext{th}_i$ are calculated using the input PDF and the NLO \texttt{APPLGRID} \cite{applgrid} interfaced with the \texttt{MCFM} parton level generator \cite{MCFM-I,MCFM-II,MCFM-III}. The NNLO accuracy is reached via $k$-factors ($kf$) calculated in each observable bin, as the ratio between the higher and lower order QCD calculation
\begin{equation}
    kf_i = \frac{\sigma_i^{NNLO}}{\sigma_i^{NLO}}.
\end{equation}
%In this formula both the NNLO and NLO term are calculated with the same PDF, in a way to factorize the PDF effects.
The NNLO DYTurbo results presented in the previous section are used to calculate the $k$-factors.

\subsection{Results} \label{sec:result-pdf-prof}
Some modern sets of PDFs are used for the comparison with the ATLAS data and using the NNLO theory predictions from DYTurbo. The PDF sets considered are NNPDF3.1$\_$nnlo$\_$as$\_$0118 \cite{nnpdf31}, NNPDF4.0 \cite{NNPDF40}, CT18NNLO, CT18ANNLO \cite{ct18nnlo} and MSHT20nnlo$\_$as118 \cite{MSHT20}.
In Table \ref{tab:prof-results-nnpdf31-nnpdf40} the $\chi^2$ results using the NNPDF3.1 and NNPDF4.0 for the comparison are reported. In table \ref{tab:prof-results-ct18-ct18a} the results using the CT18 and CT18A PDF sets are shown. Finally the results using MSHT20 PDF set are reported in Table \ref{tab:prof-results-msht20}. In each of the  result tables, the $\chi^2$ contribution from each data set, the first term on the right hand side of eq. \ref{eq:prof-chi2},  is reported, together with the corresponding number of degrees of freedom. At the bottom of the table the correlated and total $\chi^2$ are listed. Different theory predictions from DYTurbo are tested: the fixed order NNLO calculation, the prediction including the FPC term, and the $q_T$ resummed calculation. The results seem to be in line with what exposed in section \ref{sec:fiducial-power-corr}:  the data-theory agreement  improves when including the FPC term in the NNLO predictions, obtaining a reasonable $\chi^2$ over degrees of freedom. A further improvement is obtained when considering the $q_T$ resummation effects (third column in Tables \ref{tab:prof-results-nnpdf31-nnpdf40},  \ref{tab:prof-results-ct18-ct18a}, \ref{tab:prof-results-msht20}), resulting in a $\chi^2/ndf\sim 1$. This behaviour of the results is noticeable with each  of the PDF sets under consideration. 

\begin{table}[]
  \caption{Results of compariosn of the NNPDF3.1 and NNPDF4.0 PDF sets with the ATLAS 7 TeV datasets, using different NNLO theories definitions. The NNLO precision is reached with KFactor calcultated from the DYTurbo predicitons.}
\centering
\centerline{ % when the table is larger than \textwidht it expands on both sides
    \begin{tabular}{llll}
                                  & NNPDF3.1 & & \\
                                  &  NNLO   & NNLO+FPC   & NNLO+NNLL  \\
  Data set                         &      &         & \\ \hline
  ATLAS 7 TeV $y_Z$ low mass CC & 14 / 6& 9.8 / 6& 8.5 / 6  \\
  ATLAS 7 TeV $y_Z$ $Z$-peak CC  & 8.4 / 12& 6.7 / 12& 6.3 / 12  \\
  ATLAS 7 TeV $y_Z$ $Z$-peak CF  & 5.2 / 9& 5.4 / 9& 7.1 / 9  \\
  ATLAS 7 TeV $y_Z$ high mass CC  & 5.7 / 6& 5.8 / 6& 5.3 / 6  \\
  ATLAS 7 TeV $y_Z$ high mass CF  & 4.8 / 6& 4.8 / 6& 4.6 / 6  \\
  \thickhline
  Correlated $\chi^2$  & 16& 15& 9.7  \\
  Log penalty $\chi^2$  & -2.28& -2.28& -2.72  \\
  Total $\chi^2$ / dof  & 52 / 39& 45 / 39& 39 / 39  \\
  $\chi^2$ p-value  & 0.09 & 0.23 & 0.48   \\
  \hline\hline
                               & NNPDF4.0 &           &  \\
                               & NNLO        & NNLO+FPC       & NNLO+NNLL   \\
Data set                        &             &                &             \\\hline
ATLAS 7 TeV $y_Z$ low mass CC  & 15.2/6     & 10.2/6        & 8.7/6      \\
ATLAS 7 TeV $y_Z$ $Z$-peak CC & 12.1/12    & 8.3/12        & 6.5/12     \\
ATLAS 7 TeV $y_Z$ $Z$-peak CF & 9.8/9      & 5.7/9         & 7.3/9      \\
ATLAS 7 TeV $y_Z$ high mass CC & 5.1/6      & 5.7/6         & 5.3/6      \\
ATLAS 7 TeV $y_Z$ high mass CF & 4.6/6      & 5/6         & 4.8/6      \\
\thickhline
Correlated $\chi^2$            & 8.02    & 12.6     & 6.6  \\
Log Penalty $\chi^2$           & -2.1    & -1.6    & -2 \\
Total $\chi^2/$dof             & 52.7/39        & 46/39          & 37.1/39 \\
$\chi^2$ p-value               & 0.07 & 0.20 & 0.56 \\
    \end{tabular}
}

    \label{tab:prof-results-nnpdf31-nnpdf40}
\end{table}

\begin{table}[]
\caption{Results of the comparison of the CT18 and CT18A PDF sets with the ATLAS 7 TeV datasets, using different NNLO theory definitions. The NNLO precision is reached with KFactor calcultated from the DYTurbo predicitons.}
\begin{tabular}{llll}
                               & CT18 NNLO      &                    &             \\
                               & NNLO          & NNLO+FPC       & NNLO+NNLL   \\
Datasets   & & &            \\         \hline
ATLAS 7 TeV $y_Z$ low mass CC  & 7.2/6        & 5.7/6         & 5.9/6      \\
ATLAS 7 TeV $y_Z$ $Z$-peak CC & 12.6/12      & 8.3/12        & 7.1/12     \\
ATLAS 7 TeV $y_Z$ $Z$-peak CF & 8.9/9        & 6/9         & 7.2/9      \\
ATLAS 7 TeV $y_Z$ high mass CC & 5.3/6        & 5.8/6         & 5.4/6      \\
ATLAS 7 TeV $y_Z$ high mass CF & 4.6/6        & 5/6         & 4.6/6      \\
\thickhline
Correlated $\chi^2$            & 13.6      & 13.3     & 10.1  \\
Log Penalty $\chi^2$           & -3.5      & -3    & -3 \\
Total $\chi^2$                 & 48.7/39      & 41.1/39       & 36.9/39    \\
$\chi^2$  p-value  &           0.13        &       0.38   &   0.57 \\
%$\chi^2$ p-value
\hline\hline
                               & CT18A NNLO   &                   &             \\
                               & NNLO          & NNLO+FPC       & NNLO+NNLL   \\
Datasets                       &               &                &             \\\hline
ATLAS 7 TeV $y_Z$ low mass CC  & 7.4/6        & 5.9/6         & 6.1/6      \\
ATLAS 7 TeV $y_Z$ $Z$-peak CC & 12.4/12      & 8.2/12        & 6.9/12     \\
ATLAS 7 TeV $y_Z$ $Z$-peak CF & 8.7/9        & 6/9         & 7.2/9      \\
ATLAS 7 TeV $y_Z$ high mass CC & 5.4/6        & 5.7/6         & 5.5/6      \\
ATLAS 7 TeV $y_Z$ high mass CF & 4.5/6        & 5/6         & 5/6      \\
\thickhline
Correlated $\chi^2$            & 13.2      & 13.1     & 9.7  \\
Log Penalty $\chi^2$           & -3.5      & -2.9    & -3.4 \\
Total $\chi^2$                 & 48.1/39         & 41.1/39          & 36.6/39 \\
$\chi^2$ p-value               & 0.15             & 0.38              & 0.58 \\
\end{tabular}
\label{tab:prof-results-ct18-ct18a}
\end{table}

\begin{table}[]
\caption{Results of the comparisong of the MSHT20 PDF set with the ATLAS 7 TeV datasets, using different NNLO theory definitions. The NNLO precision is reached with KFactor calcultated from the DYTurbo predicitons.}
\begin{tabular}{llll}
                               & MSHT20                       &                              &                             \\
                               & NNLO                         & NNLO+FPC                     & NNLO+NNLL                   \\
Dataset                        &                              &                              &                             \\\hline
ATLAS 7 TeV $y_Z$ low mass CC  & 19.9/6                      & 12.1/6                      & 11.3/6                     \\
ATLAS 7 TeV $y_Z$ $Z$-peak CC & 14.0/12                     & 7.7/12                      & 7/12                     \\
ATLAS 7 TeV $y_Z$ $Z$-peak CF & 10.9/9                      & 6.5/9                       & 8.1/9                      \\
ATLAS 7 TeV $y_Z$ $Z$-mass CC & 5.2/6                       & 5.9/6                       & 5.3/6                      \\
ATLAS 7 TeV $y_Z$ high mass CF & 4.9/6                       & 5.3/6                       & 5.1/6                      \\
\thickhline
Correlated $\chi^2$            & 20.3                     & 15.9                   & 14.1                  \\
Log Penalty $\chi^2$           & -3.6                      & -3.1                  & -3.5                 \\
Total $\chi^2$                 & $71.7/39$ & $50.4/39$ & $47.3/39$ \\
$\chi^2$ p-value               & $0.001$    & $0.11$     & $0.17$ \\
\end{tabular}
\label{tab:prof-results-msht20}
\end{table}

\section{Conclusion and outlook}\label{sec:conclusion-pheno-study}
%NNLO QCD predictions for the Drell-Yan process have been investigated in this chapter, the results of the slicing and global subtraction methods have been taken into account. In the presence of fiducial cuts on the final state leptons, the outcome of the calculations can differ between the two methods, by an amount that is compatible with the pure NNLO correction. The fiducial cuts induce a linear dependence of the cross section on small $q_T$ values, this causes a bias in the threshold parameter of the slicing method calculations, furthermore it introduces non perturbative effect in the $q_T$-inclusive cross section and that causes instability in the convergence on the series expansion. The differences have been investigated in section \ref{sec:nlo-nnlo-benchmark}. A correction term for the linear fiducial bias has been also introduced, this takes into account for 
%The calculations, in the presence of fiducial cuts have been shown to depend on the method of the calculation. Because of fiducial cuts, a linear in the slicing parameter is introduced in the gloabl subtraction methodsglobal (or slicing) subtraction methods results are affected by a linear bias in $q_T$, the vector boson transverse momentum. Furthermore the dependance of the cross section on 
In this chapter, a study regarding high precision QCD predictions for DY was introduced and the differences between the two main calculation methods, local (or slicing) subtraction and global subtraction methods, in the presence of fiducial cuts on the final state leptons, have been explored. Some cut configurations lead the phase space acceptance to have a dependence on the vector boson transverse momentum, $q_T$, at small values. This induces linear $q_T$ biases in the slicing method predictions and furthermore introduces an instability in the convergence of the series expansion, regardless of the subtraction scheme used. In section \ref{sec:nlo-nnlo-benchmark} it has been shown how the inclusion of a fiducial power correction (FPC) term improves the nominal accuracy of the results. This correction allows us to perform benchmark comparison between global and local subtraction scheme calculations. The FPC term comes from the resummation results. The resummation program offers a way to resum the linear $q_T$ bias at each perturbative order and improves the stability of the power expansion. The downside of including resummation effect is the introduction of additional parameters in the calculation. A further investigation should include the theoretical uncertainty effects related to this new parameters. 

The theory predictions of chapter \ref{chap:pheno-study} are calculated in the same fiducial region as in the ATLAS $Z$ measurement at $7\umeas{TeV}$ \cite{atlas-w-z-7tev}, and are used in section \ref{sec:pdf-study} for a comparison study with the data. The comparison tests different PDF sets, and the various theory predictions. In particular the fixed order NNLO predictions, the prediction including the FPC term and the resummed results are tested. With the latter two, an improvement of the agreement $\chi^2$ is observed. The ATLAS collaboration performed also a $W^{+/-}$ measurement in the same analysis; to complete the picture, these data and the corresponding predictions could be added to the PDF study of section \ref{sec:pdf-study}. The results of this study is in preparation \cite{dis-22-conference,my-pubbl-fpc}.

The $q_T$ resummation effects can be important in the presence of lepton fiducial cuts. So far these effects have been ignored when determining the parton distribution functions (PDF). To fully assess the variation in the results a PDF fit should be performed varying the underlying theory and comparing the the different outcomes. The study can be a combined fit of deep inelastic scattering data from the HERA experiment \cite{H1-zeus-combination} and the most relevant Drell-Yan data sets. For some of the DY data it would be important to evaluate the effects of resummation.
%A fit can be This can be done using the DIS data from the HERA experiment \cite{H1-zeus-combination} and adding the DY data sets. 
Other than the ATLAS $W/Z$ measurements at $7\umeas{TeV}$, interesting DY measurements to include are for example the ATLAS $W/Z$ measurements at $5\umeas{TeV}$ and $8\umeas{Tev}$ \cite{atlas-wz-5tev,atlas-wz-8tev}, the CMS $W$ and $Z$ forward-backward asymmetry measurements at $7$ and $8\umeas{TeV}$ \cite{cms-z-fbasym-8tev,cms-w-fbasym-7tev} and also the Drell-Yan analysis performed at Tevatron collider by the D0 \cite{D0-DY-Zee,D0-Amu-Wmunu,D0-A_W,D0-A_e} and CDF \cite{CDF-DY-Zee-1.8TeV,CDF-DY-Zee-1.96TeV,CDF-A_W,CDF-W-Ae} experiments. 
%A PDF set obtained from the fit of DIS and the more relevant and modern Drell-Yan data represents a starting point to obtain a reference PDF set for precision EW measurement at the LHC.
